Softened Symbol Grounding for Neuro-symbolic Systems

Neuro-symbolic learning generally consists of two separated worlds, i.e., neural network training and symbolic constraint solving, whose success hinges on symbol grounding, a fundamental problem in AI. This paper presents a novel, softened symbol grounding process, bridging the gap between the two worlds, and resulting in an effective and efficient neuro-symbolic learning framework. Technically, the framework features (1) modeling of symbol solution states as a Boltzmann distribution, which avoids expensive state searching and facilitates mutually beneficial interactions between network training and symbolic reasoning;(2) a new MCMC technique leveraging projection and SMT solvers, which efficiently samples from disconnected symbol solution spaces; (3) an annealing mechanism that can escape from %being trapped into sub-optimal symbol groundings. Experiments with three representative neuro symbolic learning tasks demonstrate that, owining to its superior symbol grounding capability, our framework successfully solves problems well beyond the frontier of the existing proposals.

==> contents/delete.tex <==
% SMT solver is currently the underlying engine for practical program analysis and program verification~\citep{barnett2005boogie, cadar2008klee, godefroid2012sage},  
% ensuring that our framework can be readily extended to a broad range of application tasks. 

%However, 
%most of the existing work is often restricted or inefficient. 
%On the one hand, 
%since symbolic reasoning is non-differentiable, 
%the policy gradient methods like REINFORCE 
%become a standard approach to bridging the neural and symbolic systems~\citep{williams1992simple, liang2018memory, agarwal2019learning}. 
%Unfortunately, the sparse reward problem of these methods is nearly unavoidable, 
%which causes the training to be prohibitively unstable and inefficient. 
%On the other hand, 
%to bypass the spare reward problem, 
%one often parses the symbolic execution to derive pseudo labels that satisfy the symbolic reasoning rule~\citep{lee2013pseudo, li2020closed, tian2022weakly}.
%Nevertheless, 
%such work often needs a particular design for the parser of the given task, 
%which limits its generalizable usage. 
% Moreover, as we showed in Section~\ref{XXX}, merely utilizing pseudo labels is insufficient to train the neural network when there are quite a few feasible truth assignments for logic rules.


%In this paper, 
%we show that, in neural-symbolic learning, 
%the crucial step of solving symbol grounding problem is to identify and avoid the \emph{vacuous truth} in symbolic reasoning~\citep{XXX}. 
%For example, consider a Boolean-vector-valued variable denoted by $\s{z} \in \{T,F\}^k$ as the symbolic input, 
%and suppose that we can analyze the program and obtain all truth-assignments $\{\bm{\phi}_1, \dots, \bm{\phi}_m\}$ that can produce the target output.
%Therefore, we can equivalently formulate the weakly supervised label as the disjunctive formula $(\s{z}=\bm{\phi}_1) \vee \dots \vee (\s{z}=\bm{\phi}_m)$. 
%It should be noted that these truth-assignments are mutually exclusive, and thus the symbol grounding problem is reduced to determining whether a truth assignment $\bm{\phi}$ is the ground truth, or vacuous truth. \footnote{Strictly speaking, the vacuous truth refers to the issue that logical formula $P \to Q$ does not express its actual semantics because the antecedent $P$ cannot be satisfied.  However, the disjunction can be converted to the implication, and in our paper }

%Furthermore, 
%we also integrate the back-search proposed by~\citet{li2020closed} into our framework, 
%to accelerate the convergence when the grounding problem is initially solved. 
%Moreover, we parse the symbolic program execution based on the satisfiability modulo theories (SMT) solver~\citep{nieuwenhuis2006solving, moura2008z3, barrett2011cvc4}, which is currently the underlying engine for practical program analysis and program verification~\citep{barnett2005boogie, cadar2008klee, godefroid2012sage},  
%ensuring that our framework can be readily extended to a broad range of application tasks. 
